Empirical Analysis of Sri Lankan Mobile Health Ecosystem: A Precursor to an Effective Stakeholder Engagement

Sri Lanka recently passed its first privacy legislation covering a wide range of sectors, including health. As a precursor for effective stakeholder engagement in the health domain to understand the most effective way to implement legislation in healthcare, we have analyzed 41 popular mobile apps and web portals. We found that 78% of the tested systems have third-party domains receiving sensitive health data with minimal visibility to the consumers. We discuss how this will create potential issues in preparing for the new privacy legislation.

==> AnalysisBrainstorm.tex <==
Points of Analysis:\\

\begin{itemize}
    \item For each app...
    \begin{enumerate}
        \item for each hipaa identifier what domains received the identifier? of the receivers what percent are third party vs first party?  
        \item Is the third party open to BAA agreements e.g. Mixpanel signs BAAs but Facebook says they don't sign BAAs so don't share health data
        \item average number of third party domains communicated with? 
        \item used third party hosting/storage providers? Are the providers hipaa compliant? 
        
    \end{enumerate}
    \item For each domain...
    \begin{enumerate}
        \item how many hipaa identifiers did it receive? what were the  identifiers? delineate between first party vs third party domains.
        \item receiving X identifier, first party vs third party domain?
    \end{enumerate}
    \item Misc:
    \begin{itemize}
        \item highlight goodRX findings?
        \item How do we find out what apps correspond to a hospital that is considered a regulated entity?
        \item How do we figure out if the app has a BAA with the providers it is sharing information with?
        \item How many developers of these apps know about the "Mobile Health Apps Interactive Tool"?
        \item Look Into -> For instance, the Federal Trade Commission (FTC) Act and the FTC’s Health Breach Notification Rule (HBNR) may apply in instances where a mobile health app impermissibly discloses a user’s health information
    \end{itemize}
    
\end{itemize}

\section{Liam's Notes:}
Health apps have become increasingly popular in recent years, with many individuals using them to monitor their fitness, track their food intake, and manage chronic conditions. However, the legal background on health apps can be complex, as there are various laws and regulations that govern how personal health information can be collected, used, and shared.

In the United States, one of the most important laws that applies to health apps is the Health Insurance Portability and Accountability Act (HIPAA). HIPAA is a federal law that sets standards for the privacy and security of personal health information. If a health app is used by a "covered entity," which includes healthcare providers, health plans, and healthcare clearinghouses, then the app must comply with HIPAA regulations. This means that the app must have appropriate safeguards in place to protect the privacy and security of personal health information, and that the app must have a business associate agreement (BAA) with any third-party vendors that it shares personal health information with. This BAA must explicitly outline compliance with HIPAA rules. A BAA is a legal contract that outlines the responsibilities of the vendor in protecting the privacy and security of personal health information. "Regulated entities must ensure that all tracking technology vendors have signed a BAA and that there is an applicable permission prior to a disclosure of PHI"

If a health app is not used by a covered entity, then it is not subject to HIPAA regulations. However, other laws may still apply, such as state data breach notification laws, consumer protection laws, and the Federal Trade Commission Act.

User consent is an important aspect of HIPAA. Under HIPAA, covered entities must obtain written consent from patients before using or disclosing their personal health information for purposes other than treatment, payment, or healthcare operations. This means that if a health app is used by a covered entity, then the app must obtain user consent before collecting, using, or sharing personal health information. " Website banners that ask users to accept or reject a website’s use of tracking technologies, such as cookies, do not constitute a valid HIPAA authorization." If a health app is not used by a covered entity, then the app should still obtain user consent before collecting, using, or sharing personal health information.

Sources:

U.S. Department of Health and Human Services. Professionals. https://www.hhs.gov/hipaa/for-professionals/index.html
U.S. Department of Health and Human Services. Business Associate Contracts. https://www.hhs.gov/hipaa/for-professionals/covered-entities/sample-business-associate-agreement-provisions/index.html
U.S. Department of Health and Human Services. Privacy. https://www.hhs.gov/hipaa/for-professionals/privacy/guidance/hipaa-online-tracking/index.html

\newpage
